Wafer-Scale Fast Fourier Transforms

We have implemented fast Fourier transforms for one, two, and three-dimensional arrays on the Cerebras CS-2, a system whose memory and processing elements reside on a single silicon wafer. The wafer-scale engine (WSE) encompasses a two-dimensional mesh of roughly 850,000 processing elements (PEs) with fast local memory and equally fast nearest-neighbor interconnections. Our wafer-scale FFT (wsFFT) parallelizes a $n^3$ problem with up to $n^2$ PEs. At this point a PE processes only a single vector of the 3D domain (known as a pencil) per superstep, where each of the three supersteps performs FFT along one of the three axes of the input array. Between supersteps, wsFFT redistributes (transposes) the data to bring all elements of each one-dimensional pencil being transformed into the memory of a single PE. Each redistribution causes an all-to-all communication along one of the mesh dimensions. Given the level of parallelism, the size of the messages transmitted between pairs of PEs can be as small as a single word. In theory, a mesh is not ideal for all-to-all communication due to its limited bisection bandwidth. However, the mesh interconnecting PEs on the WSE lies entirely on-wafer and achieves nearly peak bandwidth even with tiny messages. This high efficiency on fine-grain communication allow wsFFT to achieve unprecedented levels of parallelism and performance. We analyse in detail computation and communication time, as well as the weak and strong scaling, using both FP16 and FP32 precision. With 32-bit arithmetic on the CS-2, we achieve 959 microseconds for 3D FFT of a $512^3$ complex input array using a 512x512 subgrid of the on-wafer PEs. This is the largest ever parallelization for this problem size and the first implementation that breaks the millisecond barrier.

==> txt/Compute-bound.tex <==
R = Precision in Words (1 or 2)
L = LogN
N = Size
M = SIMD MUL
A = SIMD A



=14 + 
(17 + 2R) * ((1-POWER(2;L))/-1) +
( 3*(N/A) + (N/2)/M + (N/2)/M) * L +
(L*(9+R*2+5+4*(N/A)+4) ) +
( 14L - 14 + 4 * ( (L-1)*(N/A) + 8*( (1-POWER(2;L-1)) /-1) ) )
----

= 14 + 
(17 + 2R) * ( 2^L - 1) +
L*( 3N/A + N/M ) +
L*(18 + 2R + 4N/A) +
( 14L - 14 + 4 * ( (L-1)*(N/A) + 8*2^(L-1) - 8 ) )

----

= 14 + 
(17 + 2R) * ( N - 1) +
L*( 3N/A + N/M ) +
L*(18 + 2R + 4N/A) +
14L - 14 + 4 * ( (L-1)*(N/A) + 4N - 8 )

---- FP16 (R=1, M=4, A=4)

= 14 + 
19N - 19 +
L*( 3N/4 + N/4 ) +
L*(20 + 4N/4) +
14L - 14 + 4 * ( (L-1)*(N/4) + 4N - 8 )

= 14 + 19N - 19 + L*N + L*N + 20L + 14L - 14 + 4*(L*N/4 - N/4 + 4N - 8)
---
= 19N + 2*L*N + 34L + L*N - N + 16N - 32 - 19
--
= 19N + 3LN + 34L +15N - 51
--
= 34N + L(3N + 34) - 51

---------------------------

= 14 + (17 + 2R) * ( N - 1) +
L*( 3N/A + N/M ) +
L*(18 + 2R + 4N/A) +
14L - 14 + 4 * ( (L-1)*(N/A) + 4N - 8 )

---- FP16 (R=2, M=1, A=2)
= 14 + 21 N - 21 + 
L*( 3N/2 + N ) +
L*(18 + 4 + 2N) +
14L - 14 + 4 * ( (L-1)*(N/2) + 4N - 8 )
----
= 14 + 21 N - 21 + 
L*( 5N/2 ) +
L*(22 + 2N) +
14L - 14 + 4 * ( L*(N/2) + 3.5N - 8 )
---
= -7 + 21 N + L*2.5N + 22L + 2NL +
14L - 14 + 4L*(N/2) + 14N - 32
---
= 6.5NL + 35N + 36L - 53
= 35N + L(6.5N + 36) - 53


FP16: 34N + 3NL + 34L
FP32: 35N + 6.5NL + 36L

==> txt/Proof.tex <==

We study the communication time for 3D FFTs of size $n^3$ on a square submesh of PEs where each one holds m$\times$m pencils of size $n$.
For our implementation, the PE memory capacity limits m to be no more than 2.

It is sufficient to consider one row of PEs and the links between them.
Identical communications occur on each row of the mesh.

We derive a lower bound on the time by identifying the most heavily used links (there are two) in the row of PEs, counting 
the wavelets that traverse these links, and dividing by the link bandwidth, which is one wavelet per cycle.

Let $p=n/m$ be the number of PEs in a row, numbered from 0 to p-1.
In the transpose operations, the $i^{th}$ PE sends $p-i-1$ messages towards higher-index PEs and $i$ messages towards lower-index PEs.
Each message is an m$\times$m$\times$m cube of complex numbers.

Because of the symmetry we need only consider the traffic that flows toward the last PE.
We imagine the PEs to be arranged in a line with PE 0 at the left end and $PE_{p-1}$ at the right end.
Each of the messages sent to the right is only captured by one of the router filters, and the other routers just let it flow rightwards.
The data travels all the way to $PE_{p-1}$.
Thus, the link leading into $PE_{p-1}$ from the left, carries one message from $PE_{p-2}$, two messages from $PE_{p-3}$, and so on, up to $p-1$ messages from $PE_{0}$
Therefore, this link has to transfer $p(p-1)/2$ messages.

In reality, we do not send all of the messages that traverse the last link in one uninterrupted sequence.
There are temporal gaps that add some overhead.
Once a PE has sent all the data it must, it sends a last \textit{control wavelet} to trigger a reconfiguration of the filter in the next router.
There is a delay of $d$ cycles before the next router can start sending. Since this happens at each router, and there are $p-1$ of them between the left and rightmost, it adds $d\times(p-1)$ cycles to the time.

Therefore the cycle count of a communication phase cannot be less than the bound:

cycles >= $d\times(p-1)$ (delay cycles) + $p(p-1)/2$ (messages) * $m^3$ (numbers per message) * r (cycles per number) = ($d$ + $p/2$ * $m^3$ * $r$)($p - 1$) cycles. 
Given that we use complex numbers and that the link is 32-bit wide, using FP32 data makes $r=2$, while with FP16 $r=1$.
Considering the FP32 case, the single-pencil case where $m=1$ has a runtime of ($d$ + $p$)($p - 1$) cycles.
Since $p=n/m$, the runtime with respect to problem size $n$ is  ($d$ + $n$)($n - 1$) = $n^2 + (d-1)n - d$ cycles.
The multi-pencil case where $m=2$ has a runtime of ($d$ + $8(n/2)$)($n/2 - 1$) = $2n^2 + (d/2 - 4)n - d$ cycles.
We have measured $d$ to be close to 30. 
The mesh extent $n$ is considerably larger than $d$ for our problem sizes of interest, so it still makes sense to think of this bound as roughly $n^2$ for $m=1$ and $2n^2$ for $m=2$.
Thus, cutting the mesh in half in each dimension with fixed problem size leads to roughly doubling the communication time.
%On the other hand, the compute time goes up by a factor of 4. The compute/communication balance improves.
Since $d=30$ and we only study strong scaling for $n>=256$ we know that the upper bound of the communication time with $m=2$ is $2\times$ the time of $m=1$, i.e., $(2n^2 + 11n - 30) / (n^2 + 29n - 30) <= 2$.


% (In the literature, you do not need to “show your work” when the work is algebra of this kind.   You should convince yourself it is right, then just give the bottom line result as above.)


% MARCELO:  How big an FFT would have equal compute and comm time on a 512$\times$512 mesh?    How much memory per PE would be needed?
% And if the mesh went up to 1024^2, and you ask the same question, do you get the same m and the same memory requirement, or do you need more (or less) memory per PE to have a comp/comm balance at a larger mesh size?

 

% PS – It might be better to not make R the driving thing.
% You could introduce MP, which generalizes SP and the parameter m right from the get go.
% Set the problem to be an N^3 FFT once and for all.
% Then you have R = N/m  as the mesh extent, so formulas involving R become formulas involving N and m, and they are valid once and for all in the SP and MP cases.
%You wouldn’t then have that abrupt change from R-based to N based formulas, as you do now.  

% Moreover, you might just add the multiplicative constant W for words and wavelets per complex number, setting it to 2 for FP32 and 1 for fp16.   But I don’t think you need to, we could just restrict this analysis to FP32.
% It is interesting that fp16 doesn’t buy much, since the comp time is irrelevant and the comm time has the annoying F=30 in it which doesn’t become 15 when you go to half precision.

% It’s most interesting to do the investigation of what more memory buys you.  IE back to weaker scaling.   A little bit of that (with a lot more memory than we currently have) would boost the megaflops, I guess.
% Speed costs memory.  Always has….

%---------
% Note that only a small fraction, R-1, of the numbers sent across this link are relevant to $PE_{R-1}$.
% Perhaps these relevant numbers could arrive first, allowing the PE to start the next superstep before the irrelevant data arrive.   Unfortunately,
% our implementation doesn’t allow that.   Because of the way we have programmed the routers, $PE_{R-1}$ first receives R-1 numbers from PE 0; then R-2 from PE 1, until it finally receives 1 number from PE R-2.  Thus, it takes the full R(R-1) cycles before the last relevant data are received.
% The quadratic dependence on R is best possible.
% If one considers the link in the middle of the row, it must transfer $R^2/4$ numbers from left to right, as half of the half of the data that begin in the left half of the row are sent to the right half of the row.
% Thus at two wavelets per number, even if we were to stop wavelets at their destinations, this link would have to carry $R^2/2$ wavelets.
% The fact that we do not stop them leads to the congestion at the edge, which is worse than this unavoidable bottleneck by a factor of two.
